Multi-Action Dialog Policy Learning from Logged User Feedback

Multi-action dialog policy, which generates multiple atomic dialog actions per turn, has been widely applied in task-oriented dialog systems to provide expressive and efficient system responses. Existing policy models usually imitate action combinations from the labeled multi-action dialog examples. Due to data limitations, they generalize poorly toward unseen dialog flows. While reinforcement learning-based methods are proposed to incorporate the service ratings from real users and user simulators as external supervision signals, they suffer from sparse and less credible dialog-level rewards. To cope with this problem, we explore to improve multi-action dialog policy learning with explicit and implicit turn-level user feedback received for historical predictions (i.e., logged user feedback) that are cost-efficient to collect and faithful to real-world scenarios. The task is challenging since the logged user feedback provides only partial label feedback limited to the particular historical dialog actions predicted by the agent. To fully exploit such feedback information, we propose BanditMatch, which addresses the task from a feedback-enhanced semi-supervised learning perspective with a hybrid objective of semi-supervised learning and bandit learning. BanditMatch integrates pseudo-labeling methods to better explore the action space through constructing full label feedback. Extensive experiments show that our BanditMatch outperforms the state-of-the-art methods by generating more concise and informative responses. The source code and the appendix of this paper can be obtained from https://github.com/ShuoZhangXJTU/BanditMatch.

==> algo_bm.tex <==
% \begin{wrapfigure}{L}{0.5\textwidth}
% \begin{minipage}{0.5\textwidth}
\begin{algorithm}[t]
\small
\algnewcommand{\LineComment}[1]{\State \(//\) #1}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithmic}[1]

\Require {Target policy and the logging policy parameters $\theta$ and $\theta_0$, bandit data $\mathcal{D_B} = \{(\bs_i, \hat{\bA}_i, \brho_i, \delta_i):i=1,\ldots,B\}$.} 

\Ensure {Updated target policy parameters $\theta$.}

\State Initialization:
$\theta \leftarrow \theta_0$;

\LineComment Initiate the feedback-enhanced thresholds.

\For{i=1,\ldots,B}

\State Collect the correctly-predicted positive samples $D_T$.

\EndFor

\State Compute $\btau^{Y}_{pos}$, $\btau^{N}_{pos}$, and $\text{MC}_{pos}$ by Eq. (4)-(6).

\While {Not converged}

\For{i=1,\ldots,B} 

\LineComment Update the feedback-enhanced thresholds.

\State Add the correctly-predicted positive samples to $D_T$.

\State Compute $\btau^{Y}_{pos}$, $\btau^{N}_{pos}$, and $\text{MC}_{pos}$ by Eq. (4)-(6).

\State Obtain the negative samples $B_N$.

\State Compute $MC_{neg}$ with $\pi_\theta$ and $B_N$ by Eq. (7).

\State Compute $\btau^{Y}_{neg}$ and $\btau^{N}_{neg}$ by Eq. (2) and (3).

\LineComment Feedback-enhanced semi-supervised learning.

\State Compute $\mathcal{L_L}$, $\mathcal{L_P}$, $\mathcal{L_B}$  and $\mathcal{L_K}$ by Eq. (9), (11)-(13).

\State Compute the overall loss $\mathcal{L}$ by Eq. (14).

\State Update $\theta \leftarrow \theta -\eta\nabla\mathcal{L}$.

\EndFor

\EndWhile

\end{algorithmic}  
\caption{BanditMatch algorithm.}
\label{alg1}
\end{algorithm}
% \end{minipage}
% \end{wrapfigure}
